Towards Detecting Contextual Real-Time Toxicity for In-Game Chat

Real-time toxicity detection in online environments poses a significant challenge, due to the increasing prevalence of social media and gaming platforms. We introduce ToxBuster, a simple and scalable model that reliably detects toxic content in real-time for a line of chat by including chat history and metadata. ToxBuster consistently outperforms conventional toxicity models across popular multiplayer games, including Rainbow Six Siege, For Honor, and DOTA 2. We conduct an ablation study to assess the importance of each model component and explore ToxBuster's transferability across the datasets. Furthermore, we showcase ToxBuster's efficacy in post-game moderation, successfully flagging 82.1% of chat-reported players at a precision level of 90.0%. Additionally, we show how an additional 6% of unreported toxic players can be proactively moderated.

==> comments.tex <==
============================================================================ 
ACL-Industry 2023 Reviews for Submission #71
============================================================================ 

Title: DTBERT: Detecting In-game Chat Toxicity with BERT
Authors: Zachary Yang, Yasmine Maricar, Mohammadreza Davari, Nicolas Grenon-Godbout and Reihaneh Rabbany


============================================================================
                            REVIEWER #1
============================================================================

Key Lessons
---------------------------------------------------------------------------
This paper is a fairly straightforward use of BERT for toxicity detection.  There is novelty in that the authors created a new dataset specifically aimed at their target application, which is chat during game play, and that was the primary interest in applying a BERT-based model.  The other areas that involved some novelty—or, at least, some model choices—were the inclusion of the entirety of the chat history (up to the limit of the model's block size) and the augmentation of chat turns based on speaker (essentially, annotating a form of diarization).
---------------------------------------------------------------------------


Strengths
---------------------------------------------------------------------------
The trained model does best on its own domain, beating out other off-the-shelf models that are general purpose (i.e., not trained on the domain of interest).  Of particular note is the ability of the DT-BERT model to have high recall, roughly tracking precision, unlike the results for the off-the-shelf models ("baselines") against which DT-BERT was tested.  In the appendix, however, it is clear that DT-BERT suffers its own domain-shift problem, as it performs less well compared to, say, Perspective API on Jigsaw's Toxic Comment Classification dataset.
---------------------------------------------------------------------------


Weaknesses
---------------------------------------------------------------------------
While reading the paper, there was a surprising lack of detail in describing the model itself.  In §3.2, there is a simple one-sentence natural language description that the model is a BERT model, with a pointer to Figure 1.  Only by reading Appendix C does one obtain more detail about the model itself, although there are still elements missing: Figure 1 includes a box labeled "MLP" atop the "C" token (which is presumably the [CLS] token).  What are the dimensions of that MLP?  Also, I tried to find out exactly how inference was being done.  When the authors describe token-level vs. sentence-level, I *think* they mean that the sentence-level prediction is happening by providing a softmax atop the MLP atop the [CLS] representation, but I am not sure.  And is the token-level version some aggregation function over the token representations?  Again, I couldn't find the details in the paper (I am hopeful they are there and I just missed them, but a reader shouldn't have to work !
 hard to find such details).

It is slightly unfair to present results on a new dataset, compare against more generic off-the-shelf models *without* presenting results on more established datasets at the same time.  I.e., I think the material in Table 12 ought to appear in §4 of the main paper and not in an appendix.  For one thing, the statistics in Table 6 show an inordinate amount of chat turns—two thirds—falling in the "Spam" category; is that much more prevalent than, say, in the Jigsaw dataset?

One more thing on comparison: the authors say that Perspective API is not capable of working with the entire chat history.  But how can that be?  Couldn't the authors simply have prepended as much chat history as Perspective API's or Cleanspeak's length limit would allow and evaluate the performance of Perspective API and Cleanspeak on chat turns with history prepended?  Such a comparison would be fairer.

There is no error analysis presented.  Even though DT-BERT does very well on its own domain, it would have been very helpful to see both wins and (especially) losses on the development test set.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #2
============================================================================

Key Lessons
---------------------------------------------------------------------------
This paper explored a BERT based in-game chat toxicity detection model. Chat history and metadata were leveraged and found to be able to boost model performance. The practical implication of utilizing the model in actual moderation was discussed. It was also shown that the model can successfully transfer to different games.
---------------------------------------------------------------------------


Strengths
---------------------------------------------------------------------------
This paper was well organized and clearly written. They trained a BERT based model on their toxicity data set which captured a diverse perspective, and designed experiments to test the benefits of including chat history as well as other metadata. The performance impact of including extra information were elucidated through ablation study. Mature commercial toxicity detection models were employed for comparison. Furthermore, the authors also discussed the practical implications of utilizing the model in actual moderation, covering both scientific and practical aspects of the problem.
---------------------------------------------------------------------------


Weaknesses
---------------------------------------------------------------------------
For wider application of the model, the transferability of the model to other games were investigated. However, the experiment was only done on one other game and there was no description on how different Game 2 was from Game 1. Also to show true transferability, I believe the comparison should be between model trained with Game 1 plus limited number of training data from Game 2, to model trained with only limited number of training data from Game 2. 
There are also a few typos through the paper:
1. line 049, should be "those that do report only slight improvements"? 
2. line 159, should be "the token classification task"?
3. line 191, should be "to include only"?
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #3
============================================================================

Key Lessons
---------------------------------------------------------------------------
Language between social media and in-game chat need to have different dataset. Past chat history helps to improve toxicity model performance in game-chat dataset.
---------------------------------------------------------------------------


Strengths
---------------------------------------------------------------------------
This paper proposes DTBERT for detecting in-game chat toxicity. The model incorporates chat history and speaker information.

The paper is motivated well and easy to follow.

Experiment results demonstrate the proposed model outperforms several baslines.
---------------------------------------------------------------------------


Weaknesses
---------------------------------------------------------------------------
The novelty of the paper is limited, encoding history information is common in conversational models.

It would be good to see how many past conversations are good enough to boost the model performance.

The proposed DTBERT model is trained on in-game chat data specifically, however, all the baseline models are not trained on this domain data.

Some minor issues: in abstract, it it unclear what does +7 or +57 mean. What does "DT" stand for in "DTBERT"
---------------------------------------------------------------------------

